Hardness-guided domain adaptation to recognise biomedical named entities under low-resource scenarios

Domain adaptation is an effective solution to data scarcity in low-resource scenarios. However, when applied to token-level tasks such as bioNER, domain adaptation methods often suffer from the challenging linguistic characteristics that clinical narratives possess, which leads to unsatisfactory performance. In this paper, we present a simple yet effective hardness-guided domain adaptation (HGDA) framework for bioNER tasks that can effectively leverage the domain hardness information to improve the adaptability of the learnt model in low-resource scenarios. Experimental results on biomedical datasets show that our model can achieve significant performance improvement over the recently published state-of-the-art (SOTA) MetaNER model

==> rename.tex <==
\begin{table*}[!th]
\centering
\small
\textbf{Precision Performance}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|l|cc|cc|cc|cc|}
    \hline
    \multicolumn{1}{|c|}{$\mathcal{T}^{'}$}
        & \multicolumn{1}{c|}{}
        & \multicolumn{2}{c|}{Disease} 
        & \multicolumn{2}{c|}{Drug} 
        & \multicolumn{2}{c|}{Gene} 
        & \multicolumn{2}{c|}{Species}
        % & \multicolumn{1}{c|}{Overall}
    \\ \cline{3-10}
    
    \multicolumn{1}{|c|}{Size}
        & \multicolumn{1}{c|}{}
        & NCBI & BC5CDR 
        & BC5CDR & BC4CHEMD 
        & JNLPBA  & BC2GM
        & LINNAEUS  & S800 
        
    \\ \hline 
    
    \parbox[t]{3mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{5}}}}
    &\textbf{MetaNER}
        &{0.3645}&{0.4010}&{0.7740}&{0.4048}&{0.1717}&{0.2050}&{0.6278}&{0.2589}\\

    &\textbf{BioBERT}
        &{0.0324}&{0.0305}&{0.1099}&{0.0283}&{0.0573}&{0.0489}&{0.0055}&{0.0054}\\
        
    &\textbf{HGDA}
        &{0.3937}&{0.5039}&{0.7355}&{0.4085}&{0.3175}&{0.3431}&{0.4312}&{0.3538}\\
    
    &\textbf{HGDA-NEs}
        &{0.4540}&{0.5044}&{0.7023}&{0.3203}&{0.3507}&{0.3887}&{0.5784}&{0.4551}\\

    &\textbf{HGDA*}
        &{0.2219}&{0.1419}&{0.5400}&{0.1502}&{0.2928}&{0.2616}&{0.0860}&{0.1899}\\
    
    &\textbf{HGDA-NEs*}
        &{0.3059}&{0.2203}&{0.5858}&{0.1761}&{0.2546}&{0.2571}&{0.1954}&{0.2401}\\
    
    \hline \hline
    
    \parbox[t]{3mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{10}}}}
    &\textbf{MetaNER}
        &0.3176&0.3721&0.7079&0.3398&0.2864&{0.3175}&{0.6281}&{0.3812}\\
    
    &\textbf{BioBERT}
        &{0.1038}&{0.0426}&{0.3964}&{0.0916}&{0.1608}&{0.2480}&{0.0444}&{0.0221}\\
        
    &\textbf{HGDA}
        &{0.4311}&{0.4656}&{0.7227}&{0.4457}&{0.4300}&{0.4468}&{0.4991}&{0.3714}\\

    &\textbf{HGDA-NEs}
        &{0.5715}&{0.5651}&{0.7079}&{0.4226}&{0.3762}&{0.3938}&{0.4354}&{0.3206}\\

    &\textbf{HGDA*}
        &{0.3318}&{0.3581}&{0.6324}&{0.2844}&{0.3370}&{0.3117}&{0.1264}&{0.2909}\\
    
    &\textbf{HGDA-NEs*}
        &{0.3847}&{0.3172}&{0.6815}&{0.3666}&{0.3113}&{0.2824}&{0.1452}&{0.2844}\\
    
    \hline \hline
        
    \parbox[t]{3mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{20}}}}
    &\textbf{MetaNER}
        &{0.4699}&{0.4652}&{0.7523}&{0.4384}&{0.3516}&{0.3625}&{0.5462}&{0.2611}\\
    
    &\textbf{BioBERT}
        &{0.3907}&{0.3402}&{0.7389}&{0.2518}&{0.3048}&{0.4067}&{0.1954}&{0.2362}\\
    
    &\textbf{HGDA}
        &{0.5968}&{0.5926}&{0.7846}&{0.4771}&{0.4836}&{0.4910}&{0.5205}&{0.4443}\\

    &\textbf{HGDA-NEs}
        &{0.5698}&{0.5263}&{0.7650}&{0.4680}&{0.4745}&{0.4805}&{0.7638}&{0.5419}\\
    
    &\textbf{HGDA*}
        &{0.3634}&{0.3876}&{0.6338}&{0.3660}&{0.3918}&{0.3467}&{0.1243}&{0.2787}\\
    
    &\textbf{HGDA-NEs*}
        &{0.4354}&{0.4587}&{0.7027}&{0.4173}&{0.3722}&{0.3428}&{0.2455}&{0.3205}\\
        
    \hline \hline
        
    \parbox[t]{3mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{50}}}}
        
    &\textbf{MetaNER}
        &{0.6154}&{0.6150}&{0.75}&{0.4824}&{0.4938}&{0.5030}&{0.64}&{0.3455}\\
    
    &\textbf{BioBERT}
        &{0.5661}&{0.5455}&{0.7679}&{0.4308}&{0.3963}&{0.5314}&{0.6914}&{0.4020}\\
    
    &\textbf{HGDA}
        &{0.6659}&{0.5916}&{0.8006}&{0.5734}&{0.5035}&{0.5141}&{0.7683}&{0.5911}\\
    
    &\textbf{HGDA-NEs}
        &{0.6320}&{0.5692}&{0.7722}&{0.5585}&{0.5587}&{0.5901}&{0.7331}&{0.5578}\\
    
    &\textbf{HGDA*}
        &{0.5060}&{0.5258}&{0.7083}&{0.3758}&{0.4202}&{0.3820}&{0.3580}&{0.3699}\\
        
    
    &\textbf{HGDA-NEs*}
        &{0.5536}&{0.5720}&{0.7566}&{0.5497}&{0.4971}&{0.4697}&{0.3243}&{0.3663}\\
    \hline
    \end{tabular}
\end{adjustbox}
\vspace{-2mm}
\caption{
Average precision-performance of the sequence encoder adaptation for bioNER tasks with the best performance boldfaced. All results have the same settings with those from \autoref{tab:heterogeneous}.
}
\label{tab:heterogeneous-precision}
\vspace{-5mm}
\end{table*}


\begin{table*}[!th]
\centering
\small
\textbf{Recall Performance}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|l|cc|cc|cc|cc|c|}
    \hline
    \multicolumn{1}{|c|}{$\mathcal{T}^{'}$}
        & \multicolumn{1}{c|}{}
        & \multicolumn{2}{c|}{Disease} 
        & \multicolumn{2}{c|}{Drug} 
        & \multicolumn{2}{c|}{Gene} 
        & \multicolumn{2}{c|}{Species}
        & \multicolumn{1}{c|}{Overall}
    \\ \cline{3-10}
    
    \multicolumn{1}{|c|}{Size}
        & \multicolumn{1}{c|}{}
        & NCBI & BC5CDR 
        & BC5CDR & BC4CHEMD 
        & JNLPBA  & BC2GM
        & LINNAEUS  & S800 
        &    
    \\ \hline 
    
    \parbox[t]{3mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{5}}}}
    &\textbf{MetaNER}
        &{0.2493}&{0.1689}&{0.4818}&{0.1725}&{0.3099}&{0.3196}&{0.0700}&{0.1110}&{}\\

    &\textbf{BioBERT}
        &{0.1029}&{0.1294}&{0.0828}&{0.0369}&{0.1402}&{0.0700}&{0.0932}&{0.0482}&{}\\
        
    &\textbf{HGDA}
        &{0.2780}&{0.2084}&{0.5446}&{0.2027}&{0.4580}&{0.3454}&{0.1212}&{0.2498}&{}\\
    
    &\textbf{HGDA-NEs}
        &{0.2247}&{0.1934}&{0.4852}&{0.2471}&{0.4280}&{0.3467}&{0.0947}&{0.1981}&{}\\

    &\textbf{HGDA*}
        &{0.2617}&{0.0485}&{0.4759}&{0.1251}&{0.5114}&{0.4327}&{0.0719}&{0.4199}&{}\\
    
    &\textbf{HGDA-NEs*}
        &{0.3342}&{0.1048}&{0.6442}&{0.3728}&{0.4824}&{0.4504}&{0.0498}&{0.3829}&{}\\
    
    \hline \hline
    
    \parbox[t]{3mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{10}}}}
    &\textbf{MetaNER}
        &{0.3555}&{0.3913}&{0.6381}&{0.3574}&{0.4149}&{0.3447}&{0.2052}&{0.2843}&{}\\
    
    &\textbf{BioBERT}
        &{0.1275}&{0.0970}&{0.2724}&{0.0997}&{0.2612}&{0.1973}&{0.1266}&{0.0728}&{}\\
        
    &\textbf{HGDA}
        &{0.3887}&{0.3904}&{0.6486}&{0.4135}&{0.5497}&{0.4615}&{0.2134}&{0.3802}&{}\\

    &\textbf{HGDA-NEs}
        &{0.3627}&{0.3481}&{0.6261}&{0.3996}&{0.5313}&{0.4334}&{0.1821}&{0.3341}&{}\\

    &\textbf{HGDA*}
        &{0.4631}&{0.4704}&{0.7061}&{0.4870}&{0.5799}&{0.5500}&{0.1883}&{0.5045}&{}\\
    
    &\textbf{HGDA-NEs*}
        &{0.4503}&{0.3216}&{0.7438}&{0.4740}&{0.5507}&{0.5459}&{0.1255}&{0.4733}&{}\\
    
    \hline \hline
        
    \parbox[t]{3mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{20}}}}
    &\textbf{MetaNER}
        &{0.4559}&{0.4859}&{0.7116}&{0.4460}&{0.5133}&{0.4325}&{0.4574}&{0.3574}&{}\\
    
    &\textbf{BioBERT}
        &{0.3126}&{0.2429}&{0.5582}&{0.2351}&{0.4923}&{0.4529}&{0.1290}&{0.2422}&{}\\
    
    &\textbf{HGDA}
        &{0.5362}&{0.5235}&{0.7167}&{0.5194}&{0.6315}&{0.5391}&{0.2922}&{0.4449}&{}\\

    &\textbf{HGDA-NEs}
        &{0.5418}&{0.5019}&{0.7009}&{0.4768}&{0.6135}&{0.5573}&{0.3598}&{0.5076}&{}\\
    
    &\textbf{HGDA*}
        &{0.5406}&{0.6074}&{0.7846}&{0.5911}&{0.6426}&{0.5866}&{0.2584}&{0.5503}&{}\\
    
    &\textbf{HGDA-NEs*}
        &{0.5395}&{0.5945}&{0.7717}&{0.6138}&{0.6390}&{0.6015}&{0.3563}&{0.5545}&{}\\
        
    \hline \hline
        
    \parbox[t]{3mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{50}}}}
        
    &\textbf{MetaNER}
        &{0.5382}&{0.6079}&{0.7475}&{0.5392}&{0.5825}&{0.5109}&{0.5918}&{0.3819}&{}\\
    
    &\textbf{BioBERT}
        &{0.6406}&{0.6108}&{0.7384}&{0.5691}&{0.6283}&{0.6608}&{0.5122}&{0.5379}&{}\\
    
    &\textbf{HGDA}
        &{0.5896}&{0.5982}&{0.7499}&{0.5732}&{0.6486}&{0.5792}&{0.5480}&{0.5830}&{}\\
    
    &\textbf{HGDA-NEs}
        &{0.6115}&{0.6027}&{0.7541}&{0.6024}&{0.6845}&{0.6149}&{0.5670}&{0.5361}&{}\\
    
    &\textbf{HGDA*}
        &{0.6333}&{0.6690}&{0.8172}&{0.5644}&{0.7025}&{0.6429}&{0.5883}&{0.6043}&{}\\
    
    &\textbf{HGDA-NEs*}
        &{0.6475}&{0.6764}&{0.8554}&{0.7023}&{0.7095}&{0.6563}&{0.6823}&{0.6508}&{}\\
    \hline
    \end{tabular}
\end{adjustbox}
\vspace{-2mm}
\caption{
Average recall-performance of the sequence encoder adaptation for bioNER tasks with the best performance boldfaced. All results have the same settings with those from \autoref{tab:heterogeneous}.
}
\label{tab:heterogeneous-recall}
\vspace{-5mm}
\end{table*}
